Keeping Deep Lithography Simulators Updated: Global-Local Shape-Based Novelty Detection and Active Learning

Learning-based pre-simulation (i.e., layout-to-fabrication) models have been proposed to predict the fabrication-induced shape deformation from an IC layout to its fabricated circuit. Such models are usually driven by pairwise learning, involving a training set of layout patterns and their reference shape images after fabrication. However, it is expensive and time-consuming to collect the reference shape images of all layout clips for model training and updating. To address the problem, we propose a deep learning-based layout novelty detection scheme to identify novel (unseen) layout patterns, which cannot be well predicted by a pre-trained pre-simulation model. We devise a global-local novelty scoring mechanism to assess the potential novelty of a layout by exploiting two subnetworks: an autoencoder and a pretrained pre-simulation model. The former characterizes the global structural dissimilarity between a given layout and training samples, whereas the latter extracts a latent code representing the fabrication-induced local deformation. By integrating the global dissimilarity with the local deformation boosted by a self-attention mechanism, our model can accurately detect novelties without the ground-truth circuit shapes of test samples. Based on the detected novelties, we further propose two active-learning strategies to sample a reduced amount of representative layouts most worthy to be fabricated for acquiring their ground-truth circuit shapes. Experimental results demonstrate i) our method's effectiveness in layout novelty detection, and ii) our active-learning strategies' ability in selecting representative novel layouts for keeping a learning-based pre-simulation model updated.

==> sec10_reference.tex <==
@incollection{meyer2003discrete,
  title={Discrete differential-geometry operators for triangulated 2-manifolds},
  author={Meyer, M. and Desbrun, M. and Schr{\"o}der, P. and Barr, A.},
  editor ={H.-C. Hege and K. Polthier},
  booktitle={Visualization and mathematics III},
  pages={35--57},
  year={2003},
  publisher={Springer}
}

@incollection{grandstrand:2004,
  author      = "Ove Grandstrand",
  title       = "Innovation and Intellectual Property Rights",
  editor      = "Jan Fagerberg and David C. Mowery and Richard R. Nelson",
  booktitle   = "The Oxford Handbook of Innovation",
  publisher   = "Oxford University Press",
  address     = "Oxford",
  year        = 2004,
  pages       = "266-290",
  chapter     = 10,
}

@article{salehi2021unified,
  title={A Unified Survey on Anomaly, Novelty, Open-Set, and Out-of-Distribution Detection: Solutions and Future Challenges},
  author={Salehi, M. and Mirzaei, H. and Hendrycks, D. and Li, Y. and Rohban, M. and Sabokrou, M.},
  journal={arXiv preprint arXiv:2110.14051},
  year={2021}
}

@article{pimentel2014review,
  title={A review of novelty detection},
  author={Pimentel, M. and Clifton, D. and Clifton, L. and Tarassenko, L.},
  journal={Signal Process.},
  volume={99},
  pages={215--249},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{paul2016efficient,
  title={Efficient selection of informative and diverse training samples with applications in scene classification},
  author={Paul, S. and Bappy, J. and Roy-Chowdhury, A.},
  booktitle={Proc. IEEE Inf. Conf. Image Process.},
  pages={494--498},
  year={2016},
  organization={IEEE}
}

@book{kolaczyk2014statistical,
  title={Statistical analysis of network data with R},
  author={Kolaczyk, E. and Cs{\'a}rdi, G{\'a}bor},
  volume={65},
  year={2014},
  publisher={Springer}
}

@inproceedings{zhou2014improved,
  title={Improved margin sampling for active learning},
  author={Zhou, Jin and Sun, Shiliang},
  booktitle={Proc. Chinese Conf.  Pattern Recognit.},
  pages={120--129},
  year={2014},
}

@inproceedings{xu2003representative,
  title={Representative sampling for text classification using support vector machines},
  author={Xu, Zhao and Yu, Kai and Tresp, Volker and Xu, Xiaowei and Wang, Jizhi},
  booktitle={Proc. European Conf. Inf. Retr.},
  pages={393--407},
  year={2003},
}

@inproceedings{sener2018active,
  title={Active Learning for Convolutional Neural Networks: A Core-Set Approach},
  author={Sener, Ozan and Savarese, Silvio},
  booktitle={Proc. Int. Conf.  Learn. Rep.},
  year={2018}
}

@book{networkintroduction,
  author = {Mark Newman},
  year = {2010},
  title = {Networks: An Introduction},
  publisher = {Oxford University Press}
}

@inproceedings{ebert2012ralf,
  title={Ralf: A reinforced active learning formulation for object class recognition},
  author={Ebert, Sandra and Fritz, Mario and Schiele, Bernt},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={3626--3633},
  year={2012},
}

@article{roweis2000nonlinear,
  title={Nonlinear dimensionality reduction by locally linear embedding},
  author={Roweis, Sam T and Saul, Lawrence K},
  journal={Science},
  volume={290},
  number={5500},
  pages={2323--2326},
  year={2000},
  publisher={American Association for the Advancement of Science}
}

@article{chen2009fast,
  title={Fast Approximate kNN Graph Construction for High Dimensional Data via Recursive Lanczos Bisection.},
  author={Chen, Jie and Fang, Haw-ren and Saad, Yousef},
  journal={J. Mach. Learn. Res.},
  volume={10},
  number={9},
  year={2009}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Adv. Neural Inf. Process. Syst.},
  pages={5998--6008},
  year={2017}
}

@article{shao2021ic,
  title={From IC Layout to Die Photo: {A CNN}-Based Data-Driven Approach},
  author={Shao, Hao-Chiang and Peng, Chao-Yi and Wu, Jun-Rei and Lin, Chia-Wen and Fang, Shao-Yun and Tsai, Pin-Yian and Liu, Yan-Hsiu},
  journal={IEEE Trans. Comput.-Aided Design Integr. Circuits Syst.},
  volume={40},
  number={5},
  pages={957--970},
  Month={May},
  year={2021},
  publisher={IEEE}
}

@misc{C2Cdist,
  title = {Contour-to-contour distance},
  author={Shao, Hao-Chiang},
  howpublished = {\url{https://www.mathworks.com/matlabcentral/fileexchange/75551-contour-to-contour-distance}},
}

@inproceedings{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  booktitle={Proc. Int. Conf. Learn. Rep.},
  year={2021}
}

@article{SSIM,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P and others},
  journal={IEEE Trans. Image Process.},
  volume={13},
  number={4},
  pages={600--612},
  year={2004}
}

@inproceedings{cui2019class,
  title={Class-balanced loss based on effective number of samples},
  author={Cui, Yin and Jia, Menglin and Lin, Tsung-Yi and Song, Yang and Belongie, Serge},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={9268--9277},
  year={2019}
}

@article{chang2013revisit,
  title={A revisit to support vector data description},
  author={Chang, Wei-Cheng and Lee, Ching-Pei and Lin, Chih-Jen},
  journal={Dept. Comput. Sci., Nat. Taiwan Univ., Taipei, Taiwan, Tech. Rep},
  year={2013}
}

@article{tax2004support,
  title={Support vector data description},
  author={Tax, David MJ and Duin, Robert PW},
  journal={Mach. Learn.},
  volume={54},
  number={1},
  pages={45--66},
  year={2004},
  publisher={Springer}
}

@inproceedings{lee2019overcoming,
  title={Overcoming catastrophic forgetting with unlabeled data in the wild},
  author={Lee, Kibok and Lee, Kimin and Shin, Jinwoo and Lee, Honglak},
  booktitle={Proc. IEEE/CVF Int. Conf. Comput. Vis.},
  pages={312--321},
  year={2019}
}

@article{he2019analyzing,
  title={Analyzing the Forgetting Problem in the Pretrain-Finetuning of Dialogue Response Models},
  author={He, Tianxing and Liu, Jun and Cho, Kyunghyun and Ott, Myle and Liu, Bing and Glass, James and Peng, Fuchun},
  journal={arXiv preprint arXiv:1910.07117},
  year={2019}
}

@article{li2017learning,
  title={Learning without forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  journal={IEEE Trans. Pattern Anal. Mach. Intell.},
  volume={40},
  number={12},
  pages={2935--2947},
  year={2017},
  publisher={IEEE}
}

@inproceedings{zhou2017fine,
  title={Fine-tuning convolutional neural networks for biomedical image analysis: actively and incrementally},
  author={Zhou, Zongwei and Shin, Jae and Zhang, Lei and Gurudu, Suryakanth and Gotway, Michael and Liang, Jianming},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={7340--7351},
  year={2017}
}

@inproceedings{miljkovic2010review,
  title={Review of novelty detection methods},
  author={Miljkovi{\'c}, Dubravko},
  booktitle={Proc. Int. Convention MIPRO},
  pages={593--598},
  year={2010},
}

@article{liu2013svdd,
  title={Svdd-based outlier detection on uncertain data},
  author={Liu, Bo and Xiao, Yanshan and Cao, Longbing and Hao, Zhifeng and Deng, Feiqi},
  journal={Knowledge and Inf. Syst.},
  volume={34},
  number={3},
  pages={597--618},
  year={2013},
  publisher={Springer}
}

@article{terrell1992variable,
  title={Variable kernel density estimation},
  author={Terrell, George R and Scott, David W},
  journal={Annals of Statistics},
  pages={1236--1265},
  year={1992},
  publisher={JSTOR}
}

@inproceedings{japkowicz1995novelty,
  title={A novelty detection approach to classification},
  author={Japkowicz, Nathalie and Myers, Catherine and Gluck, Mark and others},
  booktitle={Proc. Int. Joint Conf. Artif. Intell.},
  volume={1},
  pages={518--523},
  year={1995}
}

@article{yang2019gan,
  title={{GAN-OPC}: Mask optimization with lithography-guided generative adversarial nets},
  author={Yang, Haoyu and Li, Shuhe and Deng, Zihao and Ma, Yuzhe and Yu, Bei and Young, Evangeline FY},
  journal={IEEE Trans. Comput.-Aided Design Integr. Circuits Syst.},
  volume={39},
  number={10},
  pages={2822--2834},
  year={2019},
  publisher={IEEE}
}

@inproceedings{ye2019lithogan,
  title={LithoGAN: End-to-end lithography modeling with generative adversarial networks},
  author={Ye, Wei and Alawieh, Mohamed Baker and Lin, Yibo and Pan, David Z},
  booktitle={Proc. ACM/IEEE Design Autom. Conf.},
  pages={1--6},
  year={2019},
}

@article{calderara2011detecting,
  title={Detecting anomalies in people’s trajectories using spectral graph analysis},
  author={Calderara, Simone and Heinemann, Uri and Prati, Andrea and Cucchiara, Rita and Tishby, Naftali},
  journal={Comput. Vis. Image Understand.},
  volume={115},
  number={8},
  pages={1099--1111},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{sabokrou2018adversarially,
  title={Adversarially learned one-class classifier for novelty detection},
  author={Sabokrou, Mohammad and Khalooei, Mohammad and Fathy, Mahmood and Adeli, Ehsan},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={3379--3388},
  year={2018}
}

@article{mathieu2015masked,
  title={Masked Autoencoder for Distribution Estimation},
  author={Mathieu, MADEby},
  year={2015}
}

@inproceedings{abati2019latent,
  title={Latent space autoregression for novelty detection},
  author={Abati, Davide and Porrello, Angelo and Calderara, Simone and Cucchiara, Rita},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={481--490},
  year={2019}
}

@inproceedings{schlegl2017unsupervised,
  title={Unsupervised anomaly detection with generative adversarial networks to guide marker discovery},
  author={Schlegl, Thomas and Seeb{\"o}ck, Philipp and Waldstein, Sebastian M and Schmidt-Erfurth, Ursula and Langs, Georg},
  booktitle={Proc. Int. Conf. Inf. Process. Med. Imag.},
  pages={146--157},
  year={2017},
}

@inproceedings{fan2020anomalydae,
  title={AnomalyDAE: Dual autoencoder for anomaly detection on attributed networks},
  author={Fan, Haoyi and Zhang, Fengbin and Li, Zuoyong},
  booktitle={Proc. IEEE Int. Conf. Acoustics Speech Signal Process.},
  pages={5685--5689},
  year={2020},
}

@article{wang2020one,
  title={One-Class Graph Neural Networks for Anomaly Detection in Attributed Networks},
  author={Wang, Xuhong and Jin, Baihong and Du, Ying and Cui, Ping and Yang, Yupu},
  journal={arXiv preprint arXiv:2002.09594},
  year={2020}
}

@inproceedings{perera2019ocgan,
  title={Ocgan: One-class novelty detection using gans with constrained latent representations},
  author={Perera, Pramuditha and Nallapati, Ramesh and Xiang, Bing},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={2898--2906},
  year={2019}
}

@inproceedings{sung2019difference,
  title={Difference-Seeking Generative Adversarial Network--Unseen Sample Generation},
  author={Sung, Yi Lin and Hsieh, Sung-Hsien and Pei, Soo-Chang and Lu, Chun-Shien},
  booktitle={Proc. Int. Conf. Learn. Rep.},
  year={2019}
}

@article{golan2018deep,
  title={Deep anomaly detection using geometric transformations},
  author={Golan, Izhak and El-Yaniv, Ran},
  journal={arXiv preprint arXiv:1805.10917},
  year={2018}
}

@article{bergman2020classification,
  title={Classification-based anomaly detection for general data},
  author={Bergman, Liron and Hoshen, Yedid},
  journal={arXiv preprint arXiv:2005.02359},
  year={2020}
}

@article{tack2020csi,
  title={Csi: Novelty detection via contrastive learning on distributionally shifted instances},
  author={Tack, Jihoon and Mo, Sangwoo and Jeong, Jongheon and Shin, Jinwoo},
  journal={arXiv preprint arXiv:2007.08176},
  year={2020}
}

@inproceedings{li2003improving,
  title={Improving one-class SVM for anomaly detection},
  author={Li, Kun-Lun and Huang, Hou-Kuan and Tian, Sheng-Feng and Xu, Wei},
  booktitle={Proc. Int. Conf. Mach. Learn. Cybern.},
  volume={5},
  pages={3077--3081},
}

@article{an2015variational,
  title={Variational autoencoder based anomaly detection using reconstruction probability},
  author={An, Jinwon and Cho, Sungzoon},
  journal={Special Lecture on IE},
  volume={2},
  number={1},
  pages={1--18},
  year={2015}
}

@article{kliger2018novelty,
  title={Novelty detection with gan},
  author={Kliger, Mark and Fleishman, Shachar},
  journal={arXiv preprint arXiv:1802.10560},
  year={2018}
}

@article{pidhorskyi2018generative,
  title={Generative probabilistic novelty detection with adversarial autoencoders},
  author={Pidhorskyi, Stanislav and Almohsen, Ranya and Adjeroh, Donald A and Doretto, Gianfranco},
  journal={arXiv preprint arXiv:1807.02588},
  year={2018}
}

@article{settles2009active,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}

@inproceedings{lewis1995sequential,
  title={A sequential algorithm for training text classifiers: Corrigendum and additional data},
  author={Lewis, David D},
  booktitle={ACM SIGIR Forum},
  volume={29},
  number={2},
  pages={13--19},
  year={1995},
}

@article{tong2001support,
  title={Support vector machine active learning with applications to text classification},
  author={Tong, Simon and Koller, Daphne},
  journal={J. Mach. Learn. Res.},
  volume={2},
  number={Nov},
  pages={45--66},
  year={2001}
}

@inproceedings{joshi2009multi,
  title={Multi-class active learning for image classification},
  author={Joshi, Ajay J and Porikli, Fatih and Papanikolopoulos, Nikolaos},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={2372--2379},
  year={2009},
}

@article{joshi2012scalable,
  title={Scalable active learning for multiclass image classification},
  author={Joshi, Ajay J and Porikli, Fatih and Papanikolopoulos, Nikolaos P},
  journal={IEEE Trans. Pattern Anal. Mach. Intell.},
  volume={34},
  number={11},
  pages={2259--2273},
  year={2012},
  publisher={IEEE}
}

@inproceedings{kapoor2009faces,
  title={Which faces to tag: Adding prior constraints into active learning},
  author={Kapoor, Ashish and Hua, Gang and Akbarzadeh, Amir and Baker, Simon},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis.},
  pages={1058--1065},
  year={2009},
}

@article{wang2016cost,
  title={Cost-effective active learning for deep image classification},
  author={Wang, Keze and Zhang, Dongyu and Li, Ya and Zhang, Ruimao and Lin, Liang},
  journal={IEEE Trans. Circuits Syst. Video Technol.},
  volume={27},
  number={12},
  pages={2591--2600},
  year={2016},
  publisher={IEEE}
}

@article{yang2015multi,
  title={Multi-class active learning by uncertainty sampling with diversity maximization},
  author={Yang, Yi and Ma, Zhigang and Nie, Feiping and Chang, Xiaojun and Hauptmann, Alexander G},
  journal={Int. J. Comput. Vis.},
  volume={113},
  number={2},
  pages={113--127},
  year={2015},
}



@inproceedings{ying2018graph,
  title={Graph convolutional neural networks for web-scale recommender systems},
  author={Ying, Rex and He, Ruining and Chen, Kaifeng and Eksombatchai, Pong and Hamilton, William L and Leskovec, Jure},
  booktitle={Proc. ACM Int. Conf. Knowledge Discovery \& Data Mining},
  pages={974--983},
  year={2018}
}

@inproceedings{tang2015line,
  title={Line: Large-scale information network embedding},
  author={Tang, Jian and Qu, Meng and Wang, Mingzhe and Zhang, Ming and Yan, Jun and Mei, Qiaozhu},
  booktitle={Proc. Int. Conf. World Wide Web},
  pages={1067--1077},
  year={2015}
}

@article{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1310.4546},
  year={2013}
}

@article{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, William L and Ying, Rex and Leskovec, Jure},
  journal={arXiv preprint arXiv:1706.02216},
  year={2017}
}

@inproceedings{grover2016node2vec,
  title={node2vec: Scalable feature learning for networks},
  author={Grover, Aditya and Leskovec, Jure},
  booktitle={Proc. ACM Int. Conf. Knowledge Discovery and Data Mining},
  pages={855--864},
  year={2016}
}

@article{roshanfekr2020ugrwo,
  title={UGRWO-Sampling: A modified random walk under-sampling approach based on graphs to imbalanced data classification},
  author={Roshanfekr, Saeideh and Esmaeili, Shahriar and Ataeian, Hassan and Khas, Neda Maleki and Amiri, Ali},
  journal={arXiv preprint arXiv:2002.03521},
  year={2020}
}

@article{lin2018data,
  title={Data efficient lithography modeling with transfer learning and active data selection},
  author={Lin, Yibo and Li, Meng and Watanabe, Yuki and Kimura, Taiki and Matsunawa, Tetsuaki and Nojima, Shigeki and Pan, David Z},
  journal={IEEE Trans. Comput.-Aided Design Integr. Circuits Syst.},
  volume={38},
  number={10},
  pages={1900--1913},
  year={2018},
  publisher={IEEE}
}

@inproceedings{zhuo2010active,
  title={Active learning framework for post-silicon variation extraction and test cost reduction},
  author={Zhuo, Cheng and Agarwal, Kanak and Blaauw, David and Sylvester, Dennis},
  booktitle={Proc. IEEE/ACM Int. Conf. Comput.-Aided Design},
  pages={508--515},
  year={2010},
  organization={IEEE}
}

@article{sener2017active,
  title={Active learning for convolutional neural networks: A core-set approach},
  author={Sener, Ozan and Savarese, Silvio},
  journal={arXiv preprint arXiv:1708.00489},
  year={2017}
}

@inproceedings{zhang2019self,
  title={Self-attention generative adversarial networks},
  author={Zhang, Han and Goodfellow, Ian and Metaxas, Dimitris and Odena, Augustus},
  booktitle={Proc. Int. Conf. Mach. Learn.},
  pages={7354--7363},
  year={2019},
}

@inproceedings{wang2018nonlocal,
  title={Non-local Neural Networks},
  author={Wang, Xiaolong and Girshick, Ross and Gupta, Abhinav and He, Kaiming},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit.},
  pages={7794--7803},
  year={2018},
}

@article{bachlechner2020rezero,
  title={Rezero is all you need: Fast convergence at large depth},
  author={Bachlechner, Thomas and Majumder, Bodhisattwa Prasad and Mao, Huanru Henry and Cottrell, Garrison W and McAuley, Julian},
  journal={arXiv preprint arXiv:2003.04887},
  year={2020}
}

@article{de2020batch,
  title={Batch normalization biases residual blocks towards the identity function in deep networks},
  author={De, Soham and Smith, Samuel L},
  journal={arXiv preprint arXiv:2002.10444},
  year={2020}
}
